Emission activity of the Be star 60 Cygni

In this paper we present results of the spectroscopic analysis of H$\alpha$ line profile of the Be star 60 Cygni. We present time evolution of the equivalent width of the H$\alpha$ line profiles during years 1992 - 2016 and $V/R$ variation during years 1995 - 2016. We analyzed data from Ond\v{r}ejov Observatory and from BeSS Database. The circumstellar disk of the star was present twice during years 1992 - 2016 and the second cycle shows stronger emission activity. We found out that the formation of the disk takes longer time than the disk extinction (extinction is much steeper than the formation) and that there is no evident period of changes in $V/R$ variation.

==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



